Generative AI for Immersive Communication: The Next Frontier in Internet-of-Senses Through 6G

Over the past two decades, the Internet-of-Things (IoT) has become a transformative concept, and as we approach 2030, a new paradigm known as the Internet of Senses (IoS) is emerging. Unlike conventional Virtual Reality (VR), IoS seeks to provide multi-sensory experiences, acknowledging that in our physical reality, our perception extends far beyond just sight and sound; it encompasses a range of senses. This article explores the existing technologies driving immersive multi-sensory media, delving into their capabilities and potential applications. This exploration includes a comparative analysis between conventional immersive media streaming and a proposed use case that leverages semantic communication empowered by generative Artificial Intelligence (AI). The focal point of this analysis is the substantial reduction in bandwidth consumption by 99.93% in the proposed scheme. Through this comparison, we aim to underscore the practical applications of generative AI for immersive media. Concurrently addressing major challenges in this field, such as temporal synchronization of multiple media, ensuring high throughput, minimizing the End-to-End (E2E) latency, and robustness to low bandwidth while outlining future trajectories.

==> Table1.tex <==
 

\begin{table*}[ht]
\caption{Comparison of Different Papers on Streaming Technologies}
\adjustbox{max width=\textwidth}{
\centering

% Set font size and row height for the entire table
%\fontsize{14}{16}\selectfont
%\renewcommand{\arraystretch}{2}
\textcolor{blue}{
\begin{tabular}{c|l|c|c|c|c|c}
    \toprule
    {\textbf{  Category}} & {\textbf{ Paper}} & {\textbf{  Type}} & {\textbf{ Media Type}} & {\textbf{ Streaming Protocol}} & {\textbf{ Encoder / Decoder}} & {\textbf{ Design Objective}} \\
    \midrule
    \multirow{8}{*}{{ \rotatebox[origin=c]{90}{\hspace{-1.4cm}  Conventional Live Streaming}}}
    & { Lo et al. (2018) \cite{lo2018edge}} & { \acs{vod}} & { 360$^{\circ}$ video \acs{erp} frames} & { \acs{dash}} & { \acs{hevc}/H.265 codec} & { Bandwidth and latency} \\
      \cmidrule(r){2-7} 
    & { Taleb et al. (2022) \cite{taleb2022vr}} & { Live} & { 360$^{\circ}$ video \acs{erp} frames} & { \acs{webrtc}} & { \acs{avc}/H.264 codec} & { Ultra low latency} \\
      \cmidrule(r){2-7} 
    & { Chen et al. (2021) \cite{chen2021optimized}} & { Live} & { 360$^{\circ}$ video \acs{erp} tiles} & { \acs{dash}} & { \acs{avc}/H.264 codec} & { Bandwidth $>$ 50\% traditional streaming} \\
      \cmidrule(r){2-7} 
    & { Yi et al. (2020) \cite{yi2020analysis}} & { Live} & { 360$^{\circ}$ video \acs{erp} frames} & { \acs{rtmp} over \acs{http}-FLV} & { \acs{avc}/H.264 codec} & { Latency $<$ 4s for 1440p resolution} \\
     \cmidrule(r){2-7} 
    & { Park et al. (2023) \cite{park2023omnilive}} & { Live} & { Spherical to 360$^{\circ}$ video \acs{erp}} & { \acs{rtmp} over \acs{hls}} & { \acs{avc}/H.264 codec} & { Super resolution and bandwidth saving} \\
    \cmidrule(r){2-7} 
    & { Gao et al. (2024) \cite{gao2024low}} & { Live} & { 360$^{\circ}$ video \acs{erp} tiles} & { \acs{rtmp} over LL-\acs{dash}} & { \acs{avc}/H.264 codec} & { Scalability} \\
   \cmidrule(r){2-7} 
    & { De Fr{\'e} et al. (2024) \cite{de2024scalable}} & { Live} & { Head position + \acs{3d} video} & { \acs{webrtc}} & { Draco codec} & { 360ms latency for 1080p video at 3Mb/s} \\
   \cmidrule(r){2-7} 
    & { Us{\'o}n et al. (2024) \cite{uson2024untethered}} & { Live} & { Volumetric video} & { \acs{webrtc}} & { \acs{vpcc} codec} & { Optimal latency at 70Mb/s bandwidth} \\
   \midrule
    \multirow{5}{*}{{ \rotatebox{90}{\hspace{-1.4cm}  Semantic Streaming}}} 
    & { Xia et al. (2023) \cite{xia2023wiservr}} & { \acs{vod}} & { 360$^{\circ}$ video tiles} & { /} & { \acs{cnn} Encoder / Decoder} & { Reduce latency with reliable transmission} \\
   \cmidrule(r){2-7} 
    & { Ahn et al. (2024) \cite{ahn2024dynamic}} & { \acs{vod} } & { Video over text semantics} & { /} & { GPT-4 Encoder / DALLE-2 Decoder} & { Video content creation} \\
   \cmidrule(r){2-7} 
    & { Chen et al. (2024) \cite{chen2024cross}} & { \acs{vod}} & { Text, audio, image, haptics} & { /} & { \begin{tabular}[c]{@{}c@{}}\acs{gnn} Encoder/\acs{3d} generative \\ reconstruction network Decoder\end{tabular}} & { \acs{3d} object construction} \\
  \cmidrule(r){2-7} 
    & { Du et al. (2023) \cite{du2023yolo}} & { \acs{vod}} & { \acs{3d} objects through text} & { /} & { \acs{cnn} (YOLOv7) Encoder / Database Decoder} & { Optimize transmission power} \\
   \cmidrule(r){2-7} 
    & { Ours} & { Live} & {\begin{tabular}[c]{@{}c@{}} Text, video frames, temperature,\\  and haptics \end{tabular}} & { \begin{tabular}[c]{@{}c@{}}\acs{http} for semantics, \acs{mqtt} for \\ sensorial data and generated code\end{tabular}} & \begin{tabular}[c]{@{}c@{}} \acs{cnn} + \acs{rnn} + GPT-3.5 Encoder \\ GPT-4 Decoder  \end{tabular} & {  Optimize bandwidth consumption} \\
    \bottomrule 
\end{tabular}
}
}
\label{tab:stateofart}
\end{table*}

